Unlikely intersection problems for restricted lifts of p-th power

I define a morphism on $\mathbb{C}_p$ called a lift of $p$-th power if its natural restriction to the residue field of $\mathbb{C}_p$ is a $p$-th power of some morphism. This definition generalizes from the lift of Frobenius. In this paper the theory of perfectoid spaces is applied on the morphism to the Manin-Mumford conjecutre, the Mordell-Lang conjecture and the Tate-Volch conjecture.

==> 01-introduction.tex <==
\section{Introduction}
A canonical idea from algebraic geometry states that if the intersection of a curve$C$ with a countable collection of ``special” points $\{P_i\}_{i\geq 1}$ is unlikely to be large unless $C$ itself is also special in some way. Questions base on this idea are are called unlikely intersection question. For instance, Lemma~\ref{Laurent} and Lemma~\ref{final} in Chapter 1 are typical results of unlikely intersections. Ihara, Serre and Tate are some pioneers on this type of problems. For algebraic dynamical systems, one can ask, for example, suppose a curve $C\subset X$ contains infinitely many periodic points under a morphism $F:X\to X$, can we say $C$ is periodic under $F$? I am going to present three questions of unlikely intersection for algebraic dynamical system, and apply Scholze's Perfectoid theory to these questions. I have to thank Junie Xie for introducing this topic in Workshop on interactions between Model Theory and Arithmetic Dynamics in Field Institute in Toronto in 2016. My work generalizes his result in~\cite{Xie}.

Let $C_p$ be the complete field of the algebraic closed field of field of $p$-adic numbers $\overline{\Q_p}$. I will work on a special kind of endomorphism of $\Aff_{\C_p}^N$, call the \emph{restricted lift of $p$-th power}. The lift of $p$-th power is a kind of endomorphism generalize the settings of lift of Frobenius. Since the definition of such endomorphism is slightly technical I will only define lift of $p$-th power and leave the restrict condition in later section (see Section~\ref{section:3}).

Written $F$ coordinate-wise as $(F_1,F_2,\ldots,F_N)$, I assume that $F_i$s are polynomials with coefficients defined in $\C_p^\circ$, the valuation ring of $\C_p$. We say $F$ is a lift of $p$-th power if there exists $G\in\C_p^\circ[X_1,\ldots, X_N]$ and $\varpi\in\C_p^\circ$ with $|p|\leq|\varpi|<1$ for the value $|\cdot|$ on $\C_p$ such that
\[
F_i=(G_i)^p\mod \varpi\C_p^\circ.
\]
For example, $(X^p+Y^p+pXY,X^p-Y^p+pXY)$ is a lift of $p$-th power on $\Aff_{\C_p}^2$. Note this endomorphism of $\Aff_{\C_p}^2$ is also a restricted of $p$-th power.

Theory of perfectoid spaces by Scholze is one of celebrating breakthrough in math in 2010s. I use this theory on three questions, dynamical Manin-Mumford conjecture, dynamical Mordell-Lang conjecture and dynamical Tate-Volach conjecture. Let me state them one by one in the following with my results.
\subsection*{Manin-Mumford Conjecture}

What Manin-Mumford Conjecture tries to say is very close to the idea of unlikely intersections. The version of dynamical systems probably is easier to state than its original version. \cite{zhang1995} gives
\begin{conjecture}\label{conjecture:manin-mumford}
Let $F:X\to X$ be an endomorphism of a quasi-projective variety defined over $K$. Let $V$ be a subvariety of $X$. If the Zariski closure of the set of preperiodic (resp. periodic) points of $F$ contained in $V$ is Zariski dense in $V$ , then $V$ itself is preperiodic (resp. periodic).
\end{conjecture}
It basically says if a variety intersects with the periodic points of $F$ infinitely many times, then the variety is also periodic under $F$. 

The original version of Manin-Mumford conjecutre was proved by Rayanaud (see~\cite{Raynaud1983,Raynaud1983incollection}) and many others (see~\cite{Ullmo1998,Zhang1998,Buium1996,Hrushovski2001}, and \cite{PinkRoessler2004}). Baker and Hsia first proved that the dynamical Manin-Mumford conjecture is true for any line on an affine space of dimension $2$. Then, many counterexamples were given (see \cite{pazuki2010, pazuki2013, GTZ2011}, and \cite{YuanZhang2017}). However, \cite{GTZ2011} also shows the conjecture is hold for some cases, and after that many cases have been proved to be valid (see~\cite{Fakhruddin2014, GNY2018, GNY2019, GhiocaTucker2010}, and \cite{DujardinFavre2017}). Now, we believe the dynamical Manin-Mumford conjecture is only failed for some special families.

The following is my result on the dynamical Manin-Mumford conjecture. 
\begin{theorem}\label{the dynamical Manin-Mumford conjecture}
Let $V$ be a variety of $\Aff_K^N$ and $F$ is a restricted lift of $p$th power, and assume that $\bar{F}^l$ is a finite surjective morphism of $red(V)\coloneqq \bar{V}$ for some integer $l\geq 1$, i.e. $\bar{F}^l:\bar{V} \to \bar{V}$. Then, if $V\cap \Per(F)$ is dense in $V$, then $V\cap\Per(F^l)=V\cap\Per(F)$ is periodic.
\end{theorem}


\subsection*{Mordell-Lang Conjecture}
The idea of Mordell-Lang conjecture is this. Let $G$ be a semiabelian variety over $\C$ and $V$ is a subvariety of $G$. Taking an element $g$ in $G$, then $\{n\in\Z\mid ng\in V\}$ is a union of finite many arithmetic progressions, i.e.
\[
\{n\in\N\mid ng\in V\}=\cup_{i=1}^k\{a_ik+b_i\mid k\in \Z\}
\]
for some integer $a_i$ and $b_i$. A more general statement is proved by Faltings (see~\cite{Faltings}) and Vojta (see~\cite{Vojta}). Dynamical version is inspired by Ghioca and Tucker (see~\cite{GhiocaTucker2009}). Many different versions of dynamical Mordell-Lang conjecture have also been given (see~\cite{BellGhiocaTucker2010}, \cite{B-G-K-T-2012}, \cite{SilvermanBianca2013} and \cite{Xie2017}). Let me state the dynamical Mordell-Lang conjecture.
\begin{conjecture}
Let $X$ be a qusi-projective variety and $V$ be a subvariety of $X$. Let $f:X\to X$ be an endomorphism. For any $x\in X$, the set $\{n\mid f^n(x)\in V\}$ is a union of finitely many arithmetic progressions. 
\end{conjecture}

However, if we look closer to the conjecture and compare the original version with the dynamical one, we will find that the above conjecture is not complete. The $n$ in the original version can be positive and negative, so we shouldn't only consider forward orbits of a dynamical system but also backward orbits of a dynamical system. The backward orbit was asked by S.-W. Zhang and solved by Xie for lift of Frobenius. They made the following conjecture.
\begin{conjecture}\label{conjecture:inverse mordel-lang}
Let $X$ be a quasi-pojective variety over a algebraic closed field $\overline{K}$ and $F:X \to X$ be a finite endomorphism. Let $\{b_i\}_{i\geq 0}$ be a sequence of points in $X$ satisfying $F(b_i)=b_{i-1}$ for all $i\geq 1$. Let $V$ be a subvariety of $X$. Then the set ${n\geq 0\mid b_n \in V }$ is a union of finitely many arithmetic progressions.
\end{conjecture}

The condition $F(b_i)=B_{i-1}$ is called coherent condition, and we can actually made a conjecture without such condition, but there are counterexamples. For instance, consider a map $F:=(x^2,x^3):\Aff_\C^2\to\Aff_\C^2$ with $b_0=(1,1)$, and let $V$ be the diagonal of $\Aff_{\C}^2$. There are other preimages of $(1,1)$ by $F^n$ is not on the diagonal, and note that $(1,1)$ is a fixed point of $F$, so I can chose $b_{2^i}$ to be $(1,1)$ and $b_i$ to be any other preimages not on the diagonal. Then, this construction will make $\{i\mid b_i\in V\}$ not a union of infinitely many arithmetic progressions. However, this example is cheating in the sense that actually $(1,1)$ is belonging to $F^{-n}((1,1))$ for all $n$. Indeed, Theorem~\ref{finialthm} shows that if $F$ is eventually stable and $V$ is defined over the defining field of $F$, then the coherent condition is automatically satisfied. A polynomial $f$ is eventually stable, if the number of factors of $f^n$ is bounded. The eventually stable condition on an endomorphism follows the similar sense (see Definition~\ref{eventuallystable} for more details). Eventually stable doesn't exit an easy criteria. Rafe and Alon (see~\cite{RafeAlon2016}) made some conjectures about the eventual stability.

In the end, I prove a theorem similar to Xie's by generalize the endomorphism to a lift of $p$-th power.
\begin{theorem}\label{Inverse Mordelll-Lang conjecture}
Let $\{a_n\}$ be a coherent backward orbit of $a_0$ by a restricted lift of $p$th power $F$. Assume that there exists a subsequence $\{a_{n_i}\}$ contained in an irreducible subveriety $V$ with $\bar{F}^{l}(\bar{V})=\bar{V}$ for some integer $l$. We further assume that $b_0$ is algebraic. Then, we have $\{n_i\}$ is arithmetic progressive.
\end{theorem}


\subsection*{Tate-Volch Conjecture}
Tate-Volch conjecture is a relative new question in algebraic geometry by \cite{TateVoloch1996}.
\begin{conjecture}\label{conjecture: tate-voloch}
Let $A$ be a semiabelian variety over $K_v$, the complete field with respect to a valuation $v$ on $K$, and $V$ a subvariety of $A$. Then there exists $c > 0$ such that for any torsion point $x \in A$, we have either $x\in V$ or $d(x,V)>c$.
\end{conjecture}
The $d(x,V)$ is the ``distance" of the point $x$ to $V$. To avoid any complicate definition, the $d(x,V)$ is the infinite norm of $V(x)$, evaluating $x$ by plugging to the defining equations of $V$.
\cite{Scanlon1999} showed the conjecture is true over any finite extension of $\Q_p$, and \cite{Buium1996onTateVoloch} proved the conjecture is true for periodic points of any lift of Frobenius endomorphism $f:V\to V$. I prove
\begin{theorem}\label{dynamical tate-voluch conjecture}
Let $F$ be a restricted lift of $p$th power over $\mathbb{\C}_p$. Then, for any variety $V$, there exists an $\varepsilon>0$ such that, for all $x\in \Per(F)$, either $x\in V$ or $d(x,V)>\varepsilon$.
\end{theorem}

The idea of using the theory of perfectoid space is straight forward since the construction of a perfectoid space is literately a dynamical system. Let $F:X\to X$ be a restricted of $p$-th power over $\C_p$. A correspondent perfectoid space $X^{perf}$ can be created with an endomorphism $F^{perf}$ such that the following diagram commutes
\[
\begin{tikzcd}
X\arrow[r,hook]\arrow[d,"F"] & {X}^{perf}\arrow[d,"{F}^{perf}"]\\
X\arrow[r,hook] & {X}^{perf}
\end{tikzcd}
\]

The tilt of the above diagram is
\[
\begin{tikzcd}
{X}^\flat\arrow[r,hook]\arrow[d,"{F}^\flat"] & {X}^{perf,\flat}\arrow[d,"{F}^{perf,\flat}"]\\
{X}^\flat\arrow[r,hook] & {X}^{perf,\flat}
\end{tikzcd}
\]
Using the theory of perfectoid spaces, one has a topological homeomorphism $\rho$ with an important approximation lemma to pass $X^{perf}$ to $X^{perf,\flat}$ with $\rho\circ F^{perf}=F^{perf,\flat}\circ \rho$. This connect the right edges of the above two diagram. On the other side, $X$ can be reduced to $\overline{X}$, defined over the residue field of $\C_p$ with $\overline{F}\e F\mod \C_p^{\circ\circ}$, where $\C_p^{\circ\circ}$ is the maximal ideal of the valuation ring of $\C_p$. The dynamical system $(\overline{X},\overline{F})$ can be naturally embedded into $(X^\flat,F^\flat)$ since the residue field of $\C_p^{\flat}=\widehat{\overline{\F_p(t^{1/p^{\infty}})}}$ is just a subfield of $\C_p^{\flat}$. In conclusion, we have reduction and embedding on one side and topological homeomorphism on the other side to connect the two commutative diagrams. Using this framework, we can pass results that is true over a field of characteristic $p$ to its correspondent field of characteristic $0$.

Finally, let me outline this chapter. I will introduce more about the theory of perfectoid spaces in the next sections, and carefully construct our framework of perfectoid spaces carefully in the third section. The fourth section will use the framework in the second section to study the periodic points of $F$. Then, I give proof of all theorems and required lemmas in the last section.

==> chapter3main.tex <==
\chapter{Perfectoid space}
\input{chapter3/01-introduction.tex}
\input{chapter3/02_introduction_of_perfected_spaces.tex}
\input{chapter3/03-construct_our_framework.tex}
\input{chapter3/04-restrict_on_periodic_points.tex}
\input{chapter3/05-main_theorems.tex}
